Towards Practical Integrity in the Smart Home with HomeEndorser

Home automation in modern smart home platforms is often facilitated using trigger-action routines. While such routines enable flexible automation, they also lead to an instance of the integrity problem in these systems: untrusted third-parties may use platform APIs to modify the abstract home objects (AHOs) that privileged, high-integrity devices such as security cameras rely on (i.e., as triggers), thereby transitively attacking them. As most accesses to AHOs are legitimate, removing the permissions or applying naive information flow controls would not only fail to prevent these problems, but also break useful functionality. Therefore, this paper proposes the alternate approach of home abstraction endorsement, which endorses a proposed change to an AHO by correlating it with certain specific, preceding, environmental changes. We present the HomeEndorser framework, which provides a policy model for specifying endorsement policies for AHOs as changes in device states, relative to their location, and a platform-based reference monitor for mediating all API requests to change AHOs against those device states. We evaluate HomeEndorser on the HomeAssistant platform, finding that we can derive over 1000 policy rules for HomeEndorser to endorse changes to 6 key AHOs, preventing malice and accidents for less than 10% overhead for endorsement check microbenchmarks, and with no false alarms under realistic usage scenarios. In doing so, HomeEndorser lays the first steps towards providing a practical foundation for ensuring that API-induced changes to abstract home objects correlate with the physical realities of the user's environment.

==> related_works.tex <==
\section{Related Works}
\label{sec:related_works}



Prior work in smart home security has heavily focused on addressing the misuse of sensitive APIs, through improvements to the platform permission model (\eg risk-based permissions~\cite{rfep18}, functionality-based enforcement~\cite{lck+17}), providing users with runtime-context of an API access (\eg ContexIoT~\cite{jcw+17}), enforcing least privilege using context from the app's description (\eg SmartAuth~\cite{tzl+17}), and, when all else fails, forensic analysis by integrating fine-grained provenance tracking into apps (\eg ProvThings~\cite{whbg18}).  
\add{
  \trent{We have made this point already, so no need to completely relitigate.  A simple reminder with a cross-ref to the argument is sufficient.  Need the space.} At first glance, our problem may also seem to be one of over-privilege or API misuse; however, we assert that addressing this problem as API misuse by retrofitting existing defenses would be both ineffective and impractical.
  \trent{This next sentence is too much.}
That is, at the fundamental level, the problem addressed in this paper is one of a lack of {\em integrity} guarantees for high integrity AHOs, and addressing the problem by identifying and removing third-party services/apps that misuse API, but without providing app-agnostic system-wide integrity guarantees, would be be akin to providing protection, but not security, as an adversary could compromise a benign service and still violate the integrity of AHOs.
Further, the approach of removing privileges (or completely preventing third-parties from accessing AHOs) would be impractical, because several third-party integrations may truly need access to AHOs, and denying access may come at prohibitive usability costs, as we previously discussed in Section~\ref{sec:need-checks}.
Thus, \tool presents a more direct solution to the lack of integrity for AHOs in the smart home.
We now discuss other prior work across several dimensions of smart home, OS, and mobile security as they relate to \tool.
}

An alternate approach to securing shared states (including AHOs) is centralizing them and only allowing trusted third parties to modify them, as Schuster et al. explored using ``environmental situation oracles''~\cite{sst+18} or ESOs.
The ESO model is mainly geared towards providing {\em privacy} (and not integrity), \ie to prevent several parties from persistently accessing the user's private information (\eg location) to generate a shared state (\eg\ \home), by only allowing one dedicated trusted app per shared state.
The key difference between ESOs and \tools endorsement is that our approach does not require a trusted party to take upon itself the responsibility of accurately generating the value for a shared state; instead, we simply provide an endorsement policy that can {\em sanity check} a modification using approximate contextual cues.
Furthermore, as stated previously, the ESO model would break existing integrations such as IFTTT~\cite{iftttapp}, and force users to use only a single app for every state.
That is, while Schuster et al. focus on accurately generating shared states, which may require significant engineering effort to scale, we assume the practical approach of sanity checking an already generated state based on physical/local device context, which is sufficient for endorsement.


\add{


Prior work has also studied transitive problems occurring in the smart home, mostly in the context of {\em app chaining/interactions} (first identified by Surbatovich et al.~\cite{sab+17}), where the premise is that two or more applications could accidentally (or maliciously) trigger one another, putting the system in an overall unsafe state~\cite{sab+17,csk+20,ctm19,cmt18,nsq+18}.
Prior defenses against app-chaining attacks involve static analysis (\eg Soteria~\cite{cmt18}, IoTSAN~\cite{nsq+18}), or runtime rule-based enforcement (\eg IoTGuard~\cite{ctm19}).
Further, Ding and Hu demonstrated that such chains can also exploit the physical interactions among devices in the home~\cite{dh18}, and in their recent work~\cite{dhc21}, further characterize these interactions, and propose the IoTSafe system, which models and predicts application interactions at runtime~\cite{dhc21}.
\tool differs from prior work on app chains (whether or not they involve physical interactions) in two key ways.
First, prior defenses are geared towards preventing attacks that involve two apps (\ie app interaction), and {\em are not designed to defend against arbitrary API calls that modify high-integrity AHOs}, which is a complementary research goal that \tool seeks to address.
Second, prior work relies on the ability to view and/or instrument apps, while \tool is app-agnostic, and only relies on local observations of device states obtained from the platform.
This is a prudent decision, as most popular platforms do not {\em host} applications/services  (\eg\ apps in \nest~\cite{wwGoogleAssistant} and SmartThings v3~\cite{smartthingsv3}).
That is, third party services access the user's devices via the platform-API, but are hosted on their own cloud environments (\eg as serverless functions), which are beyond the view or control of the platform.
\tool's app-agnostic approach is practical and ensures effectiveness in the face of this challenge.
}

\add{
\tool relies on trusted {\em endorsement attributes}, \ie attributes that cannot be modified by the adversary through API calls, but \tool does not account for byzantine faults in devices. 
However, there is prior work in the area of validating states reported by devices, particularly the recent Peeves system by Birnbach et al.~\cite{bem19}.
Peeves generates fingerprints of device events, in the form of physical changes that they {\em cause}, which are sensed by other trusted sensors, which attest to the validity of the reported device state.
These device states that Peeves validates form the building block of \tools endorsement policies that endorse {\em higher-level}, {\em abstract} home attributes (\eg\ \home, \secstate).
Hence, \tool will benefit from the additional robustness and fault tolerance enabled by complementary approaches such as Peeves, although neither system promises byzantine fault tolerance.
However, note that \tool and Peeves validate orthogonal types of states in the home, which lie at different levels of abstraction, and hence, have distinct design goals.
That is, while Peeves focuses on sensor fingerprint accuracy and precision, \tool focuses on building expressive policies that involve a variety of device states to ensure compatibility with most end-user deployments (\ref{goal:policy}), and on realizing key reference monitor properties (\ref{goal:complete-mediation}, \ref{goal:tamperproofness}, \ref{goal:freshness}).
}








Finally, a related problem of endorsing operations has also been
explored in Android.  Android devices contain many sensors (e.g.,
camera and microphone) that apps may use if authorized.  Android
depends on users to authorize the sensors that apps may use, but a
malicious app may access a sensor at will once
authorized~\cite{comm_surv21}.  To address this problem, researchers
have explored methods to endorse authorized sensor operations by
comparing the context of the sensor operation request to authorized
contexts.  For instance, user-driven~\cite{rkm+12,ringer16ccs} access
control requires that applications use system-defined GUI gadgets
associated with particular operations to enable the system to endorse
the sensor operation associated with a user input event unambiguously.
The AWare~\cite{petracca17usenix} system enables applications to
choose their own GUI gadgets, but restrict applications to employ the
same GUI configuration (e.g, layout) to endorse a sensor operation.
The EnTrust~\cite{petracca19usenix} system extends endorsement to
include the delegation context of sensor operations processed
cooperatively.  For IoT systems, we find that state change operations
must be associated with physical events, enabling them to be endorsed
based on properties of those physical events.




